AutoInst: Automatic Instance-Based Segmentation of LiDAR 3D Scans

Recently, progress in acquisition equipment such as LiDAR sensors has enabled sensing increasingly spacious outdoor 3D environments. Making sense of such 3D acquisitions requires fine-grained scene understanding, such as constructing instance-based 3D scene segmentations. Commonly, a neural network is trained for this task; however, this requires access to a large, densely annotated dataset, which is widely known to be challenging to obtain. To address this issue, in this work we propose to predict instance segmentations for 3D scenes in an unsupervised way, without relying on ground-truth annotations. To this end, we construct a learning framework consisting of two components: (1) a pseudo-annotation scheme for generating initial unsupervised pseudo-labels; and (2) a self-training algorithm for instance segmentation to fit robust, accurate instances from initial noisy proposals. To enable generating 3D instance mask proposals, we construct a weighted proxy-graph by connecting 3D points with edges integrating multi-modal image- and point-based self-supervised features, and perform graph-cuts to isolate individual pseudo-instances. We then build on a state-of-the-art point-based architecture and train a 3D instance segmentation model, resulting in significant refinement of initial proposals. To scale to arbitrary complexity 3D scenes, we design our algorithm to operate on local 3D point chunks and construct a merging step to generate scene-level instance segmentations. Experiments on the challenging SemanticKITTI benchmark demonstrate the potential of our approach, where it attains 13.3% higher Average Precision and 9.1% higher F1 score compared to the best-performing baseline. The code will be made publicly available at https://github.com/artonson/autoinst.

==> src/figures/04-fig-metrics-description.tex <==

\begin{figure}[b!]
\centerline{
\includegraphics[
width=\columnwidth]{fig_metrics_description}
}
\caption{\todo{IMAGE with splits-based metrics demonstration}
}
\label{fig:metrics_description}
\end{figure}


==> src/figures/04-fig_ablation_weight_thetas_npoints.tex <==

\begin{figure}[t!]
\centerline{
\includegraphics[
width=.95\columnwidth]{fig_ablation_weight_thetas_npoints}
}
\caption{Influence of hyperparameters $\theta^{\text{P}}, \theta^{\text{I}}$ in~\eqref{eq:similarity_score} on distribution of instance mask proposals, as captured by the number of points per instance (horizontal axis). 
$\theta^{\text{P}}_0 = 0.5, \theta^{\text{I}}_0 = 0.1$.}
\label{fig:ablation_weight_thetas_npoints}
\end{figure}


==> src/figures/ours/03-fig-chunks-split.tex <==
\begin{figure}[t]
\centerline{\includegraphics[width=0.8\columnwidth]{src/media/vector/ours/chunks-split.pdf}}
\caption{Mock figure}
\label{fig:chunks-split}
\end{figure}


==> src/figures/ours/03-mask-merge.tex <==
\begin{figure}[t]

\centerline{\includegraphics[width=0.95\columnwidth]{src/media/vector/ours/mask_merge.pdf}}
\caption{\emph{Top}: original camera image from KITTI dataset~\cite{geiger2012we}. \emph{Middle}: instance labels from SAM model~\cite{kirillov2023segment}. \emph{Bottom}: less granular mask, generated using IoU between smaller and larger bounding boxes}

\label{fig:mask-merge}
\end{figure}


==> src/main/01-intro.tex <==


\section{Introduction}
\label{sec:intro}

% 1. central role of annotated point cloud datasets for understanding large outdoor 3D scenes
% - used for real-time semantic perception so actually each point must be labelled
% - need fine-grained scene understanding i.e. accurately distinguish categories
Operation of autonomous systems in real outdoor conditions involves continuously interpreting sensor data representing their 3D environment; commonly, an initial stage involves 3D segmentation, constructing a semantics- or instance-aware environment map, ideally defined in any spatial location and at each step in time. 
% of spatially extended, dynamic outdoor 
% continuously updated constructing and maintaining a 
% to infer affordances 
Making use of progress in sensing equipment, panoptic 3D LiDAR segmentation~\cite{milioto2020lidar,behley2021benchmark} conveniently provides such a holistic environment description by densely assigning semantic and instance labels to individual 3D points. 
% State-of-the-art scene understanding methods are enabled by training deep neural networks on large annotated collections of high-quality 3D data
Recently, large collections of 3D point clouds with dense, high-quality annotations have enabled training effective panoptic 3D segmentation methods~\cite{marcuzzi2023mask,li2022panoptic,li2023cpseg} powered by deep neural networks (NNs). 


\input src/figures/01-fig-teaser
% 2. why obtaining such datasets is difficult 
% - 3D annotation is known to take longer time compared to 2D annotation
% - varying data quality (sparcity, occlusions) hard to recognise objects
Unfortunately, obtaining and, most importantly, annotating such datasets is significantly time- and labour-consuming~\cite{behley2019semantickitti, huang2019apolloscape, dai2017scannet, yeshwanthliu2023scannetpp} as 3D objects are difficult to recognize and accurately segment in sparse and noisy 3D LiDAR scans.
Recognizing this, recently proposed 3D instance segmentation approaches~\cite{peng2023openscene, takmaz2023openmask3d, kontogianni2023interactive, yue2023agile3d} seek to minimize dependence on annotated collections by integrating advanced machine learning methods. 
% seek instead attempting to generate 3D  segmentations automatically, \eg, by 
% Compared to 2D labeling (e.g. photos), annotating 3D data generally requires a larger number of actions; additionally, noise, sparcity, and occlusions inherent in LiDAR 3D point scans hamper recognition of objects and assignment of fine-grained semantic labels. 
% 3. summarise what are the possible ways to improve this
% (a) using advanced annotation tools: 
% Advanced labelling tools~\cite{wang2019latte,li2020sustech} aim to streamline annotation by enabling cross-examining information from other modalities (e.g., aligned RGB images), still predominantly relying on manual processing of 3D data.
 % has the potential to improve performance but requires extended annotation times.
% A promising path for reducing the annotation effort is to avoid labeling entire scenes from scratch, instead extending or correcting initial segmentations obtained automatically, \eg, by a machine learning method. 
% (b) initialise from X (weak manual labels, pretrained nets, domain transfer)
Naively using neural models optimized on existing labeled collections~\cite{huang2023segment3d}, however, is suboptimal due to variations in sensor configurations and acquisition conditions across datasets.
Despite this mismatch in data distributions being addressed by domain adaptation methods~\cite{bevsic2022unsupervised} to some extent, automatically adding new semantic classes remains impossible. 
% \LAURENZ{is there a grammer mistake in this sentence? I can't really understand the first part}
Approaches based on active or weakly-supervised learning~\cite{unal2022scribble,shi2022weakly} enable using sparse or incomplete labels but commonly need user input to guide initial predictions.
Very recently, distilling segmentation foundational models has seen interest for indoor domain~\cite{guo2023sam,yang2023sam3d,huang2023segment3d,peng2023learning} but remains in its infancy for outdoor LiDAR data~\cite{liu2024segment}.
% 1. Req: annotation is hard -> want an **unsupervised** (panoptic/semantic) instance segmentation method
% immediate consequences: 
%  - bc it is unsupervised, there is no way one could understand what should be an instance (no instance examples are given) (in this sense similar to (deep) clustering)
%  - this enables adapting to instances with varying granularity required for respective downstream tasks
In this work, we take an alternative path and develop an automatic learning-based algorithm for instance-based segmentation of 3D LiDAR point clouds, requiring no semantic or instance annotations during training and focusing on dense aggregated scans.
As a result, instance segmentations produced by our method are class-agnostic; to implement various downstream tasks, they can be mapped to respective class nomenclatures and instance granularities. 



% 2. Design decision: need dense point clouds
% rationale: 
%  - thus, to maximize usability/flexibility, choose to generate instances at fine-grained level (i.e. spatially "large" as well as spatially "small"), glueing close nearby instances is kinda easy
%  - smaller instances only seen on denser point clouds
% immediate consequences: 
%  - operate on static objects
%  - for memory/compute reasons, operate on local crops/chunks 
%  - local chunks -> merging algorithm + scalability
%  - facilitates image-pointcloud correspondences (can use image-based features)
We make two key design decisions leading to important implications for our method. 
First, instead of processing single scans as done by most existing approaches~\cite{nunes2022unsupervised,milioto2020lidar,marcuzzi2023mask}, we follow the common practice for manual labeling~\cite{behley2019semantickitti} and operate with \textit{dense registered 3D LiDAR acquisitions} to facilitate our algorithm to produce universally useful, high-quality instance segmentations. 
By improving the sampling density of the scanned 3D environment, this enables segmenting instances with smaller linear dimensions (\eg, vegetation or traffic signs) more reliably. 
We generally choose to produce finer granularity instances at a given sampling density, as merging these is significantly easier compared to splitting. 
Dense 3D point clouds additionally benefit dense image-to-point correspondences, enabling effective use of image-based features, but require addressing several important issues. 
We exclude dynamic objects (such as moving cars or humans) which lead to noisy instances, focusing on segmenting static environments instead.
To enable processing spatially extended 3D environments represented by billions of data points~\cite{behley2019semantickitti,fong2022panoptic}, we predict instances in local overlapping point chunks and design a scalable merging algorithm for fusing predictions obtained in each chunk. 
% To reduce memory and compute requirements



% 3. Design decision: need self-supervised features 
% rationale: we want to leverage strong features proposed recently 
% immediate consequences: 
%  - need feature proposal step reasonably merging features
%  - probably going to be noisy, so need also refinement -> self-training step
As our second design choice, drawing inspiration from the recent line of work targeting image and 3D indoor domains~\cite{wang2023cut,rozenberszki2023unscene3d,zhang2023freepoint}, we design our framework to operate in two stages: \textit{unsupervised generation and self-trained refinement of mask proposals.} 
For generation of our instance mask proposals, we integrate recently proposed deep self-supervised point-\cite{nunes2023temporal} and image-based~\cite{oquab2023dinov2} representations constructed from aligned 3D LiDAR and image captures, providing dense 3D features with high predictive power.
Combining these descriptors with spatial prior results in a weighted proxy-graph connecting scanned 3D points; cutting this graph~\cite{shi2000normalized} produces initial, possibly noisy, instance segmentations.
To eliminate spurious or noisy instances and maximize segmentation performance, we refine initial mask proposals by performing self-training using a procedure similar to~\cite{wang2023cut,rozenberszki2023unscene3d,zhang2023freepoint}.



% 4. Outcome: method for generating class-agnostic instance segmentations
%  - learning based so builds on 
%  - we adapt to segmentations suitable for common benchmarks 
%  - outperforms sota, including wrt annotation-aware measure 
We evaluate our algorithm on SemanticKITTI~\cite{behley2019semantickitti}, mapping our segmentations to ground-truth instances. 
To quantify advantages of our learning-based algorithm, we compare it to non-learnable~\cite{mcinnes2017hdbscan,yang2023sam3d}, and learnable unsupervised~\cite{nunes2022unsupervised} and supervised~\cite{marcuzzi2023mask} instance segmentation baselines.
We assess contributions of individual components and identify an optimal configuration of features for learning-based instance generation and refinement. 
% In addition to using conventional instance-based performance measures, we assess the potential of our algorithm according to a annotation-related performance measure. \AK{to be removed}
% While precise cost of such annotation is difficult to assess due to differences in annotaiton tools, X and Y measures represent suitable proxies. 
% \todo{sneak peak on our quant. results}
We contribute:
\begin{itemize}
\item A learning-based algorithm for unsupervised instance-based segmentation of outdoor LiDAR 3D point clouds. 
\item We compare multiple options to build an optimal configuration of self-supervised features for label-free generation and refinement of instance masks, achieving state-of-the-art results against multiple baselines.
\end{itemize}
% до нас :
% не исследовалось, какой набор self-sup фичей является эффективным для генерации пропозалов
% не проводился рефайнтмен пропозалов
% не оценивалось влияние на аннотацию



% Like existing clustering-based approaches~\cite{mcinnes2017hdbscan} \todo{cite more}, our algorithm predicts class-agnostic instance segmentations without ground-truth 3D annotations; however, it significantly improves segmentation performance by integrating learning-based methods within instance proposal generation and refinement steps.
% Unlike 3DUIS~\cite{nunes2022unsupervised} our method performs an additional self-training step, significantly improving performance.



% 4. our goal: develop an annotation-free method for 3D segmentation of lidar point clouds
% - free: does not require any annotations -- use pre-trained self-sup nets; 
% - class-agnostic: support arbitrary class nomenclatures
% - flexibly sized instances: operate on dense registered point clouds (for annotation not real-time) can propagate labels to single-scan point clouds
% - (as a consequence of previous) use chunks to handle complex large scale data - needs merging 
% - annotator friendly: tries to minimize number of correction ops (splits/merges)
% Differently from most conventional approaches that operate on a single LiDAR scan commonly lacking contextual information, our method operates on multiple registered acquisitions forming a denser 3D point cloud, enabling our algorithm to distinguish challenging 



% ****************************** 25.02.24 ****************************** %






% % 1. central role of annotated point cloud datasets for understanding large outdoor 3D scenes
% % - used for real-time semantic perception so actually each point must be labelled
% % - need fine-grained scene understanding i.e. accurately distinguish categories
% Operation of autonomous systems in real outdoor conditions involves continuously interpreting sensor data capturing their 3D environment; commonly, an initial stage is the 3D segmentation producing a semantics-aware environment map, ideally defined in any spatial location and at each step in time. 
% % of spatially extended, dynamic outdoor 
% % continuously updated constructing and maintaining a 
% % to infer affordances 
% Making use of progress in sensing equipment, LiDAR panoptic 3D segmentation~\cite{milioto2020lidar,behley2021benchmark} conveniently provides such a holistic environment description by densely assigning semantic and instance labels to individual 3D points. 
% % State-of-the-art scene understanding methods are enabled by training deep neural networks on large annotated collections of high-quality 3D data
% Recently, effective panoptic 3D segmentation methods were demonstrated by training deep neural networks on large collections of 3D point clouds with dense, high quality annotations~\cite{marcuzzi2023mask,li2022panoptic,li2023cpseg}. 



% % 2. why obtaining such datasets is difficult 
% % - 3D annotation is known to take longer time compared to 2D annotation
% % - varying data quality (sparcity, occlusions) hard to recognise objects
% Unfortunately, obtaining and, most importantly, annotating such datasets is well-known to be significantly time- and labour-consuming \todo{cite}. 
% Compared to 2D labeling (e.g. photos), annotating 3D data generally requires a larger number of actions; additionally, noise, sparcity, and occlusions inherent in LiDAR 3D point scans hamper recognition of objects and assignment of fine-grained semantic labels. 
% % 3. summarise what are the possible ways to improve this
% % (a) using advanced annotation tools: 
% Advanced labelling tools~\cite{wang2019latte,li2020sustech} aim to streamline annotation by enabling cross-examining information from other modalities (e.g., aligned RGB images), still predominantly relying on manual processing of 3D data.
%  % has the potential to improve performance but requires extended annotation times.


% A promising path for reducing the annotation effort is to avoid labeling entire scenes from scratch, instead extending or correcting initial segmentations obtained automatically, \eg, by a machine learning method. 
% % (b) initialise from X (weak manual labels, pretrained nets, domain transfer)
% Naively producing initial masks by using neural models optimized on existing labeled collections \todo{cite}, however, is suboptimal due to variations in sensor configurations and acquisition conditions  across datasets.
% Despite such discrepancies in scanned data distributions can to some extent be addressed by domain adaptation methods~\cite{bevsic2022unsupervised,kong2023conda,shaban2023lidar}, automatically adding new semantic classes remains impossible. 
% Approaches based on active or weakly-supervised learning~\cite{unal2022scribble,unal2023discwise} enable using sparse or incomplete labels but commonly need user input to both guide initial predictions and refine resulting masks.
% Very recently, distilling segmentation foundational models has seen interest for indoor domain~\cite{guo2023sam,yang2023sam3d,huang2023segment3d,peng2023learning} but remains in its infancy for outdoor LiDAR data~\cite{liu2024segment}.



% % 4. our goal: develop an annotation-free method for 3D segmentation of lidar point clouds
% % - free: does not require any annotations -- use pre-trained self-sup nets; 
% % - class-agnostic: support arbitrary class nomenclatures
% % - flexibly sized instances: operate on dense registered point clouds (for annotation not real-time) can propagate labels to single-scan point clouds
% % - (as a consequence of previous) use chunks to handle complex large scale data - needs merging 
% % - annotator friendly: tries to minimize number of correction ops (splits/merges)
% In this work, we aim to investigate , and propose  and design an algorithm for unsupervised instance-based segmentation of outdoor LiDAR 3D point clouds. 
% Like other unsupervised approaches~\cite{mcinnes2017hdbscan,nunes2022unsupervised}, our algorithm does not require ground-truth 3D annotations during training; instead, it relies on unsupervised generation and self-trained refinement of mask proposals. 
% As a result , our method is class-agnostic and therefore supports arbitrary class nomenclatures. 

% Differently from most conventional approaches that operate on a single LiDAR scan commonly lacking contextual information, our method operates on multiple registered acquisitions forming a denser 3D point cloud, enabling our algorithm to distinguish challenging 


% while such methods do not have a priori knowledge of target space, being class agnostic helps to be generic 


% we additionally consider its use for generating 3D instances for use in annotation
% not only can PC-level masks be easily propagated to individual scans, but also they enable adapting to instances of various class taxonomies and varying granularity at appropriate choice of hyperparameters.
% we additionally design and assess quality of our masks according to a annotation-correlated performance measure.


% % 5. summarise and compare our approach to this
% We draw inspiration from the recent line of work targeting indoor domain~\cite{rozenberszki2023unscene3d,zhang2023freepoint} and design our framework to operate in two stages. 
% We start with generation of instance mask proposals, where we extract multi-modal geometric, semantic, and color features for individual . 
% integrating them in a unified graph 


% % ; unlike these, our method perform an additional self-training step, significantly improving performance.



% % 6. sneak peak on our results
% Unlike 
% While precise cost of such annotation is difficult to assess due to differences in annotaiton tools, X and Y measures represent suitable proxies. 

% We contribute:
% \begin{itemize}
% \item A learning-based algorithm for unsupervised instance-based segmentation of outdoor LiDAR 3D point clouds. 
% \item To enable our methods, we investigate various approaches to constructing multi-modal features 
% \end{itemize}
% % до нас :
% % не исследовалось, какой набор self-sup фичей является эффективным для генерации пропозалов
% % не проводился рефайнтмен пропозалов
% % не оценивалось влияние на аннотацию





% % 1. We can scan quite large real environments using e.g. LIDAR sensors
% % 2. In a number of applications (e.g. digital content creation, urban analytics/smart cities), obtaining a detailed semantic model of the environment is crucial 
% % 3. actually, annotation for 3d is too expensive so lets try unsupervised
% % 4. detailed models mean both high-level object segmentations and fine-grained part understanding
% % 5. then, we require denser samples but accumulate them in an offline fashion
% % 6. having dense point clouds leads us to operate on more local manageable fragments/chunks
% % 7. we aggregate lots of self-supervised features into a joint point descriptor, then propose instances, then refine instances, then merge
% % 8. as a core comparison, we show comparisons vs. other unsupervised methods
% % 8. as a core comparison, we show comparisons vs. other unsupervised methods
% % 8. as a core comparison, we show comparisons vs. other unsupervised methods
% % 9. as an additional result, we also show comparisons vs. supervised/distillation methods 

% \ALEXEY{requirements for method
% (1) unsupervised, i.e. no GT labels -> use pre-trained self-sup nets; 
% (2) can reliably extract both large and smaller-size instances -> dense sampling but process chunks 
% }

% % Scene semantics on lidars is important and actively developing
% Scene semantic understanding plays a pivotal role in the seamless operation of autonomous systems. The dynamic evolution of 3D scanning technologies, exemplified by LiDARs, has markedly enhanced the capabilities of autonomous systems in comprehending their surroundings. While, on the one hand, it allows to get 3D representation of the world, on the other, semantic segmentation of collected data opens new difficulties — captured point clouds are sparse and have not regular density. To address this challenge, numerous recent works have introduced learnable approaches and architectures to increase quality and performance of semantic and panoptic segmentation for real-time onboard operation. 

% % Issues in manual labelling and existing semi-supervised approaches: manual labeling is heavy and requires a lot of human resources and trained specialist, different geographical regions -- are source of different set of classes, domain transfer issue between different sensor configurations (amount of sensors).

% To develop those methods, labeled datasets of target environments are required.  The process of manually labeling LiDAR point clouds is labor-intensive and demands substantial human resources along with specialized training. As a consequence, the efficiency of this approach is limited by the extensive time and expertise required. Furthermore, the diverse range of geographical regions and seasonal variations introduces a multitude of semantic classes and distinct object forms. Additionally, the domain transfer problem emerges when transitioning between various sensor configurations, for example using existing benchmark data, specifically concerning the quantity of beams in LiDAR sensors.

% % To automatize this process the next approaches were introduced blabla

% What approaches can automate this process: 
% \begin{enumerate}
%     \item pre-trained networks on other datasets -- issues with domain adoptation and exotic/target-specific objects
%     \item semi-supervised approaches, weakly supervised approaches -- also requires specialists and manual labeling \AK{more issues?}
%     \item unsupervised approaches -- clustering aka DBSCAN or 3DUSIP
% \end{enumerate}

% We focus on the last approach that does not require point cloud manual labeling and exploit image-based features/masks \AK{TBD} and point cloud instance segmentation based on it. Image-based domain has more developed labeled corpus in comparison to released point cloud datasets, also covers more variety of captured scenes. In this paper, we propose mechanism for transffering image-based instances (learnable/self-supervised features -- \AK{TBD}) to point cloud domain, as well as refinement of obtained labels using self-supervised network. The result is an approach for class-agnostic instance segmentation of point clouds that doesn't exploit manual labeling of point clouds

% \AK{Add somewhere that image instance segmentation is easier than point cloud labeling}

% \AK{Open-world Instance Segmentation}

==> src/main/02-related.tex <==
\section{Related Work}
\label{sec:related}


\input src/figures/03-fig-method-overview

\paragraph{Panoptic~\cite{milioto2020lidar,behley2021benchmark} and Instance~\cite{zhang2020instance} 3D Segmentation} 
% 1. where the task was introduced and where it is first explored for 3D lidar data
% Panoptic~\cite{milioto2020lidar,behley2021benchmark} and instance~\cite{zhang2020instance} 3D LiDAR segmentation are 
these are key 3D computer vision tasks with vast applications in autonomous robotics, where they serve to partition an input point cloud into distinct object instances and (panoptic only) background regions.
% Relevant for identifying and tracking objects, 
Earlier approaches produce instances by spatially clustering~\cite{zhao2022divide,mcinnes2017hdbscan} segmentations predicted by pretrained scene understanding models  but crucially depend on the performance of the backbone~\cite{choy20194d,zhu2021cylindrical}.
% 2. single scans/realtime, supervised, learned and non-learned 
% 3. multi scans/offline, supervised, learned and non-learned 
For realtime operation of mobile robots, learning-based methods have been proposed for panoptic~\cite{milioto2020lidar, sirohi2021efficientlps, gasperini2021panoster, hong2021lidar, zhou2021panoptic, li2022panoptic, marcuzzi2023mask, lai2023spherical, wu2023point, li2023cpseg} and instance-based~\cite{zhang2020instance,milioto2019fast} segmentation of single-scan 3D acquisitions.
Alternatively, segmentation of dense 3D point clouds (similar to this work) can aid annotation of 3D data or perform scene analytics. 
Here, static indoor scenes have seen the most progress with the emergence of panoptic~\cite{Narita2019PanopticFusionOV,wu2021scenegraphfusion,kolodiazhnyi2023oneformer3d} and instance~\cite{chen2021hierarchical,vu2022softgroup,sun2023superpoint,schult2023mask3d,lu2023query} understanding schemes; however instance-based segmentation of dense outdoor LiDAR 3D data remains almost unexplored~\cite{yang2021tupper}. 

% proposal-based~\cite{yang2019learning}, grouping-based~\cite{chen2021hierarchical}, and recent transformer-based techniques~\cite{schult2023mask3d, lu2023query}. 
% Some methods~\cite{yang2019learning, schult2023mask3d} report their performance on large-scale outdoor dataset for dense semantic segmentation STPLS3D~\cite{chen2022stpls3d}~--- aerial photogrammetry dataset. 
% But this data domain differs a lot from case of dense aggregated LiDAR point cloud resulting in weak generalization~\cite{huang2023segment3d}. 
All these approaches are supervised and require large-scale annotated 3D LiDAR datasets~\cite{behley2019semantickitti,fong2022panoptic}. 
We adopt a recent architectural solution~\cite{marcuzzi2023mask} in our proposal refinement network.
% Our self-trained proposal refinement network has MaskPLS 


\paragraph{Weakly-, Semi-, and Self-Supervised 3D Segmentation} 
% 4. single scans/realtime, <less/un>supervised
% 5. multi scans/offline, <less/un>supervised
% weakly supervised stuff
% semi/self supervised stuff
% domain adaptation stuff
Multiple works construct and utilize sparse annotations (\eg, a single click or a scribble per instance)~\cite{shi2022weakly,unal2022scribble}, or perform self-supervised pre-training of representations coupled with supervised fine-tuning for respective tasks~\cite{nunes2023temporal,nunes2022segcontrast}. 
Still, they predominantly target either only semantic segmentation~\cite{nunes2022segcontrast,shi2022weakly,unal2022scribble} or only indoor scenes~\cite{jiang2021guided,xu2020weakly,zhang2021perturbed,chibane2022box2mask}.
A recent domain adaptation method~\cite{bevsic2022unsupervised} transfers a pre-trained panoptic model between source and target domains, minimizing gap between them. 
None of these methods can handle new object types emerging during the inference stage.
Weakly- and semi-supervised methods can to some extent reduce the requirements for annotations but are unable to exclude them entirely. 
We integrate self-supervised point embeddings~\cite{nunes2023temporal} in our instance proposal stage.
% , unbalanced classes and the presence of unknown objects further complicate matters within this category~\cite{nunes2022unsupervised}. 



\paragraph{Unsupervised 3D Segmentation}
% , Class-Agnostic 3OpenVocabulary/2D-to-3D
To avoid the need for annotated 3D data and enable integrating object types unseen during training, multiple approaches opt to generate and refine 3D instance proposals without associated semantic labels (\ie, \textit{class-agnostic).}
Many such approaches originate from clustering algorithms and use various point cloud representations including raw 3D points~\cite{klasing2008clustering}, radial projections and range images~\cite{himmelsbach2010fast, korchev2013real, bogoslavskyi2016fast, zermas2017fast}, voxel grids~\cite{douillard2011segmentation, behley2013laser}, curved voxels~\cite{park2019curved}, \etc. 
Recently, unsupervised pointwise features~\cite{nunes2022segcontrast} were explored as a starting representation for clustering~\cite{nunes2022unsupervised}. 
To ease segmentation of above-ground objects, several methods start with ground extraction~\cite{himmelsbach2010fast, zermas2017fast, paigwar2020gndnet}; likewise, our approach integrates a robust ground estimator~\cite{lee2022patchwork++} for this purpose. 
We compare to a recent unsupervised method~\cite{nunes2022unsupervised} in our experiments.

% Usage of multi-modal data for class-agnostic instance segmentation gains more and more attention since it gives more fine-grained scene understanding than only spatial clustering. Existing works are mainly 

For the indoor domain, recent methods~\cite{rozenberszki2023unscene3d,zhang2023freepoint} propose generating 3D instance proposals using spatial proximity and color similarity, and refining proposed masks by a self-trained neural network~\cite{schult2023mask3d}; our work is conceptually similar but targets outdoor 3D LiDAR data. 
Building on the advanced representation capabilities of CLIP~\cite{radford2021learning}, \textit{open-vocabulary} semantic~\cite{peng2023openscene} and instance~\cite{takmaz2023openmask3d} segmentation of 3D indoor scans were proposed.
Multiple recent approaches~\cite{yang2023sam3d, guo2023sam, huang2023segment3d} distill 2D segmentation foundational models~\cite{kirillov2023segany}, transferring instances predicted in a set of images to 3D space. 
Among these, we compare to a simple mask merging baseline~\cite{yang2023sam3d}.


% \paragraph{Instance Annotation for 3D Segmentation}
% There are two main types of annotations for point clouds — 3D bounding boxes to split on-road instances and points-wise annotations that highlight full scene semantics.

% The main effort in acceleration of labeling process for point clouds was done for 3D bounding boxes, aiming to decrease such metrics as average time and amount of actions per instance box. 
% A variety of tools proposes one-click segmentation of instances and bounding box adjustment including approaches that are based on spatial clustering~\cite{monica2017multi}, usage of semantic maps from images~\cite{wang2019latte}, as well as  NN-based segmentations with denoising techniques~\cite{arief2020sane}. 
% Since from raw point cloud it is difficult to differ some objects visually, such tools as 3D-BAT~\cite{zimmer20193d}, SusTECH~\cite{li2020sustech}, labelCloud~\cite{sager2022labelcloud} propose solution focused on user-friendly multi-modal visualizations and enhancements in interaction with tool for bounding boxes. 

% Acceleration of full panoptic labeling is not tackled a lot from tooling point of view. 
% The major panoptic datasets for outdoor such as KITTI~\cite{behley2019semantickitti} and nuScenes~\cite{fong2022panoptic} exploited fully manual point-wise labeling. 
% In order to speed up annotations, the process of ScanNet~\cite{dai2017scannet}, ScanNet++~\cite{yeshwanthliu2023scannetpp}, ApolloScape dataset~\cite{huang2019apolloscape} labeling uses oversegmented point clouds based on spatial and normal proximity and normalized cut algorithm, then semantic and instance labels are assigned to patches. 
% \AK{In our work we are aiming to generate more sophisticated patches.}

% Recent interactive 3D instance segmentation approaches~\cite{kontogianni2023interactive, yue2023agile3d} aim to speed up 3D instance segmentation using clicks to discriminate objects from background but still require extensive manual interaction.



% \paragraph{Unsupervised 2D and 3D features} \todo{Description of approaches to get unsupervised features, motivation TARL and Dinov2 choice}



% Supervised category of those methods includes classical learning methods for semantic and panoptic segmentation (\cite{marcuzzi2023mask,lai2023spherical,wu2023point}), which are trained on established datasets and benchmarks (\cite{behley2019semantickitti,fong2022panoptic}). Challenges within this category involve domain transfer issues across diverse scenes and scenarios, particularly with rare classes. Semi-supervised and weakly-supervised approaches, such as those proposed in (\cite{shi2022weakly, jiang2021guided, xu2020weakly, zhang2021perturbed, nunes2023temporal, nunes2022segcontrast}, require annotation of a specified quantity of data ($1/5/10/50 \%$) and primarily address recognized classes. However, these methods do not adequately handle objects that emerge solely during the inference stage. Unbalanced classes and the presence of unknown objects further complicate matters within this category. Unsupervised approaches for LiDAR instance segmentation (class-agnostic approaches), that do not exploit any point cloud label information originate from clustering algorithms. Different representations of point clouds were proposed: 3D points domain~\cite{klasing2008clustering}, radial projections and range images~\cite{himmelsbach2010fast, korchev2013real, bogoslavskyi2016fast, zermas2017fast}, voxel grids~\cite{douillard2011segmentation, behley2013laser}, curved voxels~\cite{park2019curved}. Some of proposed methods first extract ground to ease segmentation of other objects~\cite{himmelsbach2010fast, zermas2017fast, paigwar2020gndnet}. Some approaches use learning in unsupervised manner, for example ~\cite{nunes2022unsupervised} exploits unsupervised SegContrast features~\cite{nunes2022segcontrast}. 

% Unsupervised approaches for instance segmentation (class-agnostic approaches), that do not exploit any point cloud label information originate from clustering algorithms. Different representations of point clouds were proposed: 3D points domain~\cite{klasing2008clustering}, radial projections and range images~\cite{himmelsbach2010fast, korchev2013real, bogoslavskyi2016fast, zermas2017fast}, voxel grids~\cite{douillard2011segmentation, behley2013laser}, curved voxels~\cite{park2019curved}. Some of proposed methods first extract ground to ease segmentation of other objects~\cite{himmelsbach2010fast, zermas2017fast, paigwar2020gndnet}. Some approaches use learning in unsupervised manner, for example ~\cite{nunes2022unsupervised} exploits unsupervised SegContrast features~\cite{nunes2022segcontrast}. 


% Monica et al.~\cite{monica2017multi} proposed instance annotation in several clicks of couple control points and automatically performs instance segmentation of neighborhood graph based on shortest path tree between those points. LATTE~\cite{wang2019latte} proposed a one-click technique for instance segmentation, that projects semantic image labels produced by Mask-RCNN and performs refinement based on spatial clustering via DBSCAN, as well as automatically calculate 3D box for segmented points. In order to improve noisy pre-segmentations on boundaries, SaNE~\cite{arief2020sane} proposed to exploit PointNet-based segmentation with custom penalization to drop noisy points from bounding boxes. Since from raw point cloud it is difficult to differ some objects visually, such tools as 3D-BAT~\cite{zimmer20193d}, SusTECH~\cite{li2020sustech}, labelCloud~\cite{sager2022labelcloud} were focused on user-friendly multi-modal visualizations and enhancments in interaction with tool. Another way for click-based annotation was proposed by Kontogianni et al.~\cite{kontogianni2023interactive} — user generates positive (for object point) and negative clicks (for background points), then, based on this information, Minkowski-based network perform online adaptation for segmentation.


% \AK{TODO: revisit those papers} Known/unknown objects: -- special embedding space ~\cite{wong2020identifying}, ~\cite{deng2023elc} --- ellipsoidal clustering and known/unknown objects, the same eval as in 3DUIS, ~\cite{hu2020learning} -- check.


% Survey -- \cite{zhao2021technical}.

% \paragraph{Image knowledge distillation}
% \cite{vobecky2022drive} -- SLidr, \cite{sautier2022image}, \cite{liu2023segment}, \cite{mahmoud2023self}

% \paragraph{Image-based features}

% \paragraph{Self-training refinement} \cite{zhang2023freepoint} - FreePoint   
% \cite{rozenberszki2023unscene3d} - Unscene3D    
% \cite{zhang2023towards} - Oyster

% % \section{Related Work}
% % \label{sec:related}

% % \paragraph{Instance Segmentation of LiDAR 3D Point Clouds}



% % \paragraph{Unsupervised 3D Semantic and Instance Segmentation}



% % \paragraph{Self-Supervised Representations and Self-Training}
% % With the advent of self-supervised (particularly, contrastive~\cite{jaiswal2020survey}) learning, effective visual representations could be learned from images without the need for image-level or dense annotations.
% % We follow this practice in our method, building on available pre-trained self-supervised models for generating initial instances.
% % Specifically, we use DINOv2~\cite{oquab2023dinov2} is a state-of-the-art image representation model based on visual transformers~\cite{dosovitskiy2020image}, and TARL~\cite{nunes2023temporal}, a point-based representation learning method pre-trained for LiDAR point  clouds~\cite{behley2019semantickitti}. 
% % % The model is trained on a large-scale dataset with a contrastive loss, enabling it to excel at extracting strong patchwise-features for different scenes as demonstrated by \cite{rozenberszki2023unscene3d}. 
% % % TARL~\cite{nunes2023temporal} is a point-based method for semantic segmentation of outdoor point clouds that is pre-trained on the KITTI dataset \cite{behley2019semantickitti}. 
% % % The pre-training scheme of TARL \cite{nunes2023temporal} is based on performing clustering on an aggregated point cloud, allowing to associate instances in consecutive lidar acquisitions to formulate a contrastive loss objective. 
% % % Due to this, TARL \cite{nunes2023temporal} provides strong 3D features for differentiating between instances. 

% % In contrast to TARL \cite{nunes2023temporal} and Dinov2 \cite{oquab2023dinov2}, SAM \cite{kirillov2023segany} is a state of the art supervised model that was trained on a large-scale 2D image segmentation dataset. 
% % SAM \cite{kirillov2023segany} is able to segment images at an instance and sub-instance level, providing accurate 2D masks that we can use for pseudo-label generation. 
% % As SAM \cite{kirillov2023segany} is trained on a labeled dataset, pseudo-masks generated using its labels can not be categorized as unsupervised. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% version of Anastasiia

% \section{Related Work}
% \label{sec:related}

% \paragraph{Panoptic and Instance 3D LiDAR Segmentation} 
% The objective of 3D scene segmentation is to partition the scene's point cloud into semantically meaningful regions or distinct objects. 

% % 1. where the task was introduced and where it is first explored for 3D
% % 2. single scans/realtime, supervised
% % 3. multi scans/offline, supervised


% % \input src/figures/03-fig-method-overview

% \paragraph{Unsupervised Instance-Based 3D LiDAR Segmentation} 

% % 4. single scans/realtime, <less/un>supervised
% % 5. multi scans/offline, 4. multi scans/offline, supervised


% % For outdoor data, especially for single LiDAR scans a set of methods was proposed to separate instances. 

% \textbf{Single LiDAR scans} Real-time LiDAR panoptic segmentation is key task in autonomous driving to operate and understand environment and agents behaviour. Fully supervised methods for semantic and panoptic segmentation~\cite{marcuzzi2023mask, lai2023spherical, wu2023point} are being actively developed, while require annotated large-scale datasets~\cite{behley2019semantickitti,fong2022panoptic}. To decrease amount of labeled data, weakly supervised and semi-supervised methods~\cite{shi2022weakly, jiang2021guided, xu2020weakly, zhang2021perturbed, nunes2023temporal, nunes2022segcontrast} were proposed. However, these methods do not adequately handle objects that emerge solely during the inference stage, unbalanced classes and the presence of unknown objects further complicate matters within this category~\cite{nunes2022unsupervised}. To deal with this, class-agnostic and unsupervised approaches are used originate from clustering algorithms. Different representations of point clouds were proposed to describe feature space: 3D points domain~\cite{klasing2008clustering}, radial projections and range images~\cite{himmelsbach2010fast, korchev2013real, bogoslavskyi2016fast, zermas2017fast}, voxel grids~\cite{douillard2011segmentation, behley2013laser}, curved voxels~\cite{park2019curved}. Some of proposed methods first extract ground to ease segmentation of other objects~\cite{himmelsbach2010fast, zermas2017fast, paigwar2020gndnet}. Some approaches use learning in unsupervised manner, for example ~\cite{nunes2022unsupervised} exploits unsupervised SegContrast features~\cite{nunes2022segcontrast}. 

% \textbf{Dense point clouds} Segmentation of dense point clouds of outdoor can ease generation of labels for LiDAR data (for example pre-label aggregated LiDAR point clouds) of as well as perform scene analytics. Dense point cloud segmentation had significant development in last years for indoor domain, exploiting proposal-based~\cite{yang2019learning}, grouping-based~\cite{chen2021hierarchical}, and recent transformer-based techniques~\cite{schult2023mask3d, lu2023query}. Some methods~\cite{yang2019learning, schult2023mask3d} report their performance on large-scale outdoor dataset for dense semantic segmentation STPLS3D~\cite{chen2022stpls3d}~--- aerial photogrammetry dataset. But this data domain differs a lot from case of dense aggregated LiDAR point cloud resulting in weak generalization~\cite{huang2023segment3d}. Some fresh works propose weakly-supervised approaches~\cite{kontogianni2023interactive, yue2023agile3d} that require user clicks to differ instance and background points as positive and negative feedback for instance segmentation network in order to speed up segmentation process but still depends on user input.

% Our task lies in between of those two domains~--- we are interested in instance segmentation for aggregated LiDAR scans in order to get semantically significant patches to ease process of labeling. 

% \paragraph{Tools for 3D labeling}
% There are two main types of annotations for point clouds — 3D bounding boxes to split on-road instances and points-wise annotations that highlight full scene semantics.

% The main effort in acceleration of labeling process for point clouds was done for 3D bounding boxes, aiming to decrease such metrics as average time and amount of actions per instance box. A variety of tools proposes one-click segmentation of instances and bounding box adjustment including approaches that are based on spatial clustering~\cite{monica2017multi}, usage of semantic maps from images~\cite{wang2019latte}, as well as  NN-based segmentations with denoising techniques~\cite{arief2020sane}. Since from raw point cloud it is difficult to differ some objects visually, such tools as 3D-BAT~\cite{zimmer20193d}, SusTECH~\cite{li2020sustech}, labelCloud~\cite{sager2022labelcloud} propose solution focused on user-friendly multi-modal visualizations and enhancements in interaction with tool for bounding boxes. 

% Acceleration of full panoptic labeling is not tackled a lot from tooling point of view. The major panoptic datasets for outdoor such as KITTI~\cite{behley2019semantickitti} and nuScenes~\cite{fong2022panoptic} exploited fully manual point-wise labeling. In order to speed up annotations, the process of ScanNet~\cite{dai2017scannet}, ScanNet++~\cite{yeshwanthliu2023scannetpp}, ApolloScape dataset~\cite{huang2019apolloscape} labeling uses oversegmented point clouds based on spatial and normal proximity and normalized cut algorithm, then semantic and instance labels are assigned to patches. \AK{In our work we are aiming to generate more sophisticated patches.}




% \paragraph{Class-agnostic/OpenVocabulary/2D-to-3D}

% Usage of multi-modal data for class-agnostic instance segmentation gains more and more attention since it gives more fine-grained scene understanding than only spatial clustering. Existing works are mainly focused on indoor domain though. 

% Unseen3D~\cite{rozenberszki2023unscene3d} proposes method that generates instance proposals, based on points spatial proximity and color similarity, and refines proposed masks with self-training NN based on Mask3D~\cite{schult2022mask3d}. FreePoint~\cite{zhang2023freepoint} also exploits pre-clustering strategy for instance proposals and weak supervision in order to refine them. OpenScene~\cite{peng2023openscene} creates scene representations at the point level, with text and image pixels co-embedded in the CLIP feature space mostly focusing on semantic segmentation. To extend this approach to instance level, OpenMask3D~\cite{takmaz2023openmask3d} forecasts class-agnostic 3D instance masks based on Mask3D~\cite{schult2022mask3d} and combines features for each mask through multi-view fusion of CLIP-based image embeddings. Set of approaches are focused on SAM foundation model~\cite{kirillov2023segment} for 2D instance segmentation and propose different techniques to transfer predicted instances to 3D space, merging with spatial clustering~\cite{yang2023sam3d}, building graph based on points similarity along with graph-NN to gain robustness in instance split~\cite{guo2023sam}, as well using two-stage training approach~\cite{huang2023segment3d}~--- for single RGB-D scan and full 3D map. 

% In our work, we focus on outdoor data specifics and use similar strategies to generate instance proposals and refine them using self-supervised NN.

% \paragraph{Unsupervised 2D and 3D features} \todo{Description of approaches to get unsupervised features, motivation TARL and Dinov2 choice}

% % Supervised category of those methods includes classical learning methods for semantic and panoptic segmentation (\cite{marcuzzi2023mask,lai2023spherical,wu2023point}), which are trained on established datasets and benchmarks (\cite{behley2019semantickitti,fong2022panoptic}). Challenges within this category involve domain transfer issues across diverse scenes and scenarios, particularly with rare classes. Semi-supervised and weakly-supervised approaches, such as those proposed in (\cite{shi2022weakly, jiang2021guided, xu2020weakly, zhang2021perturbed, nunes2023temporal, nunes2022segcontrast}, require annotation of a specified quantity of data ($1/5/10/50 \%$) and primarily address recognized classes. However, these methods do not adequately handle objects that emerge solely during the inference stage. Unbalanced classes and the presence of unknown objects further complicate matters within this category. Unsupervised approaches for LiDAR instance segmentation (class-agnostic approaches), that do not exploit any point cloud label information originate from clustering algorithms. Different representations of point clouds were proposed: 3D points domain~\cite{klasing2008clustering}, radial projections and range images~\cite{himmelsbach2010fast, korchev2013real, bogoslavskyi2016fast, zermas2017fast}, voxel grids~\cite{douillard2011segmentation, behley2013laser}, curved voxels~\cite{park2019curved}. Some of proposed methods first extract ground to ease segmentation of other objects~\cite{himmelsbach2010fast, zermas2017fast, paigwar2020gndnet}. Some approaches use learning in unsupervised manner, for example ~\cite{nunes2022unsupervised} exploits unsupervised SegContrast features~\cite{nunes2022segcontrast}. 

% % Unsupervised approaches for instance segmentation (class-agnostic approaches), that do not exploit any point cloud label information originate from clustering algorithms. Different representations of point clouds were proposed: 3D points domain~\cite{klasing2008clustering}, radial projections and range images~\cite{himmelsbach2010fast, korchev2013real, bogoslavskyi2016fast, zermas2017fast}, voxel grids~\cite{douillard2011segmentation, behley2013laser}, curved voxels~\cite{park2019curved}. Some of proposed methods first extract ground to ease segmentation of other objects~\cite{himmelsbach2010fast, zermas2017fast, paigwar2020gndnet}. Some approaches use learning in unsupervised manner, for example ~\cite{nunes2022unsupervised} exploits unsupervised SegContrast features~\cite{nunes2022segcontrast}. 


% % Monica et al.~\cite{monica2017multi} proposed instance annotation in several clicks of couple control points and automatically performs instance segmentation of neighborhood graph based on shortest path tree between those points. LATTE~\cite{wang2019latte} proposed a one-click technique for instance segmentation, that projects semantic image labels produced by Mask-RCNN and performs refinement based on spatial clustering via DBSCAN, as well as automatically calculate 3D box for segmented points. In order to improve noisy pre-segmentations on boundaries, SaNE~\cite{arief2020sane} proposed to exploit PointNet-based segmentation with custom penalization to drop noisy points from bounding boxes. Since from raw point cloud it is difficult to differ some objects visually, such tools as 3D-BAT~\cite{zimmer20193d}, SusTECH~\cite{li2020sustech}, labelCloud~\cite{sager2022labelcloud} were focused on user-friendly multi-modal visualizations and enhancments in interaction with tool. Another way for click-based annotation was proposed by Kontogianni et al.~\cite{kontogianni2023interactive} — user generates positive (for object point) and negative clicks (for background points), then, based on this information, Minkowski-based network perform online adaptation for segmentation.


% % \AK{TODO: revisit those papers} Known/unknown objects: -- special embedding space ~\cite{wong2020identifying}, ~\cite{deng2023elc} --- ellipsoidal clustering and known/unknown objects, the same eval as in 3DUIS, ~\cite{hu2020learning} -- check.


% % Survey -- \cite{zhao2021technical}.

% % \paragraph{Image knowledge distillation}
% % \cite{vobecky2022drive} -- SLidr, \cite{sautier2022image}, \cite{liu2023segment}, \cite{mahmoud2023self}

% % \paragraph{Image-based features}

% % \paragraph{Self-training refinement} \cite{zhang2023freepoint} - FreePoint   
% % \cite{rozenberszki2023unscene3d} - Unscene3D    
% % \cite{zhang2023towards} - Oyster

% % % \section{Related Work}
% % % \label{sec:related}

% % % \paragraph{Instance Segmentation of LiDAR 3D Point Clouds}



% % % \paragraph{Unsupervised 3D Semantic and Instance Segmentation}



% % % \paragraph{Self-Supervised Representations and Self-Training}
% % % With the advent of self-supervised (particularly, contrastive~\cite{jaiswal2020survey}) learning, effective visual representations could be learned from images without the need for image-level or dense annotations.
% % % We follow this practice in our method, building on available pre-trained self-supervised models for generating initial instances.
% % % Specifically, we use DINOv2~\cite{oquab2023dinov2} is a state-of-the-art image representation model based on visual transformers~\cite{dosovitskiy2020image}, and TARL~\cite{nunes2023temporal}, a point-based representation learning method pre-trained for LiDAR point  clouds~\cite{behley2019semantickitti}. 
% % % % The model is trained on a large-scale dataset with a contrastive loss, enabling it to excel at extracting strong patchwise-features for different scenes as demonstrated by \cite{rozenberszki2023unscene3d}. 
% % % % TARL~\cite{nunes2023temporal} is a point-based method for semantic segmentation of outdoor point clouds that is pre-trained on the KITTI dataset \cite{behley2019semantickitti}. 
% % % % The pre-training scheme of TARL \cite{nunes2023temporal} is based on performing clustering on an aggregated point cloud, allowing to associate instances in consecutive lidar acquisitions to formulate a contrastive loss objective. 
% % % % Due to this, TARL \cite{nunes2023temporal} provides strong 3D features for differentiating between instances. 

% % % In contrast to TARL \cite{nunes2023temporal} and Dinov2 \cite{oquab2023dinov2}, SAM \cite{kirillov2023segany} is a state of the art supervised model that was trained on a large-scale 2D image segmentation dataset. 
% % % SAM \cite{kirillov2023segany} is able to segment images at an instance and sub-instance level, providing accurate 2D masks that we can use for pseudo-label generation. 
% % % As SAM \cite{kirillov2023segany} is trained on a labeled dataset, pseudo-masks generated using its labels can not be categorized as unsupervised. 





==> src/main/acknowledgments.tex <==
\section*{Acknowledgements}

\todo{add Acknowledgements here, e.g. mention about KI Data Tooling grant}

==> src/main/old/03.1-overview.tex <==
\subsection{Overview}
\label{method:overview}

Our approach to constructing 3D instance segmentations comprises four main stages.
We start by transforming a fixed number of 3D LiDAR scans into a shared reference frame and extracting local $w \times h \times d$ chunks from the aggregated point cloud. \ALEXEY{what about 2D images?}
Next, we generate an initial set of semantic 3D instances independently in each chunk by computing per-point features using pre-trained image- and point-based representation models, constructing a weighted proxy-graph connecting points with feature-dependent edges, and performing cuts on this graph to isolate groups of points as instances.
We refine this initial set of instances in a series of self-training iterations using a point-based neural network (NN). 
\ALEXEY{what about merging predictions from disjoint chunks?}
 


==> src/main/old/03.2-data-preprocessing.tex <==
\subsection{Data Preprocessing}

To tackle fine-grained 3D instance segmentation, we represent the 3D scene by a dense, color-equipped 3D point cloud. 
In simulations, this point cloud can be obtained by dense virtual 3D scanning; in real-world scenarios, it can be obtained by aligning consecutive 3D LiDAR scans. To obtain these dense point clouds, we use all the scans within a mapping sequence (e.g. all scans from a sequence in the KITTI \cite{behley2019semantickitti} dataset).

Directly processing large-scale, noisy LiDAR point clouds at a scene level is computationally infeasible; instead, we opted to perform instance proposal generation and network training using local, overlapping point-sampled chunks. 
We build these by sampling chunk centers along estimated trajectory spaced 10\,m apart, then selecting scan points within 25$\times$25$\times$25\,m$^3$ axis-aligned square centered at the center. 
Defining an overlap between chunks serves as data augmentation, allowing to improve scene-level segmentation by merging per-chunk predictions.

To speed up operations on chunks, we apply voxel downsampling, reducing point count from $\sim$1M in raw chunks to $\sim$2K in downsampled chunks.
We found the voxel size $r = 35$\, cm to be a good tradeoff providing both high geometric detail and segmentation performance. 





==> src/main/old/03.2-pseudo-label-gen.tex <==
\subsection{Generating 3D Pseudo-Instances}
\label{method:pseudo}



We aim to create strong initial pseudo-masks, leveraging multi-modal image and point-based features. 
To enable pseudo-annotation, we construct a weighted proxy-graph by connecting 3D points with edges integrating 2D self-supervised features from Dinov2 \cite{oquab2023dinov2}, 2D supervised instance labels from SAM \cite{kirillov2023segany} as well as 3D features from TARL \cite{nunes2023temporal}.
Therefore, we make use of TARL \cite{nunes2023temporal} and Dinov2 \cite{oquab2023dinov2} features to generate unsupervised pseudo-labels and compare their performance to pseudo-annotations that additionally exploit SAM \cite{kirillov2023segany} labels.


\paragraph{Spatial Isolation and Ground Segmentation}
Points $p$ and $q$ are more likely to belong to the same instance if they are acquired in nearby spatial locations.
We capture this natural \textit{spatial proximity prior} by a coordinate-dependent weight $w_{\text{spat.}}(p, q; \theta_{\text{spat.}}) = \exp \{-\theta_{\text{spat.}} ||p - q||^2\}$ with $\theta_{\text{spat.}} > 0$. 
To make this spatial relation more explicit, we associate each scanned point with either a ground or a non-ground part of our point cloud and process respective parts separately, yielding two sets of pseudo-instances. 
\ALEXEY{give examples of classes belong to ground/non-ground parts? why do we need multiple classes for ground?} 
Handling each part independently allows to better tune parameters of the proposal generation procedure;
% weight of different features, as well as the minimum and maximum number of instances
in particular, isolating above-ground regions (e.g., vehicles) increases the spatial separation between respective point sets, providing a strong prior for more accurate clustering.
We use Patchwork++~\cite{lee2022patchwork++}, a state-of-the-art point cloud segmentation model, to identify ground regions. \ALEXEY{how? is this a binary, per-point segmentation with no postprocessing?}. \CEDRIC{We do so by using both XYZ coordinates and the intensity information of the pointcloud to obtain a binary mask. To filter noisy point segmentations we additionally drop points that are above $0.2m$ of the mean ground height.}
Both types of regions are fused back together after proposal generation. 



\paragraph{3D Point-Based Features}
We use the 3D backbone of the pre-trained TARL model~\cite{nunes2023temporal} to extract 96-dimensional point embeddings in each LiDAR scan (not the aggregated point cloud).
For compatibility with the sparse convolutional backbone~\cite{choy20194d}, input points are quantized during preprocessing; to propagate the output feature vectors to each of the original points, we assign them the features of their closest Euclidean neighbors among the quantized points.
Finally, we compute embeddings for points in the downsampled chunk by aggregating TARL embedding vectors from each local LiDAR scan and averaging embeddings over scanned points within the radius~$r = 35$\,cm to each point in the downsampled chunk.
We express similarity between points~$p$ and~$q$ by an embedding distance-dependent weight 
$w_{\text{point}}(p, q; \theta_{\text{point}}) = \exp \{-\theta_{\text{point}} ||\psi(p) - \psi(q)||^2\}$, where $\theta_{\text{point}} > 0$ and $\psi(p) \in \mathbb{R}^{96}$ is the TARL feature. 



\paragraph{Image-Based Features}
While point embeddings explicitly use the information available in the 3D space, they rely on sparse LiDAR scanning, potentially missing fine-grained geometric details in the scene.
We thus complement these embeddings with image-based features extracted from a pre-trained DINOv2~\cite{oquab2023dinov2} and SAM~\cite{kirillov2023segany} models, leveraging correspondences between points visible in each of the registered RGB photos. 


\CEDRIC{on Dinov2 part :  As \cite{oquab2023dinov2} is a VIT-based model \cite{dosovitskiy2020image}, it consists of stacked transformer decoders \cite{vaswani2017attention}, which allows us to extract low-level features on multiple levels. Inspired by the findings of \cite{keetha2023anyloc} we found the features of layer $10$ to be the most suitable. As Dinov2 processes the input image without any downscaling, we increase the patch size for larger resolution input images due to memory limitations. @Haifan please add the reasoning about exact feature being used (query/key/value, etc.)} \ALEXEY{explain how these are computed by invoking NNs on RGB photos} Those image-based features need to be projected onto visible 3D points in the respective non-ground chunk downsampled with voxelsize $0.05m$. \LAURENZ{is it enough like this? details on chunk are now explained in the section before this one}\ALEXEY{explain actually what chunks mean and how large it is, qualitatively}. 
To do this, we first retrieve the timestamps where scan-positions \LAURENZ{change to: where the corresponding positions from either SuMA poses (\cite{behley2018rss}, KITTI) or ground-truth positions (NuScenes)}\ALEXEY{what is this} fall into the spatial chunk borders.
For each visible timestamp we first perform mesh-based hidden point removal (HPR) using meshes generated with Make It Dense \cite{vizzo2022ral}.\todo{give more details}
This is followed by reprojecting visible points to the 2D frame and then applying the instance ids (SAM) and the feature vectors (Dinov2) onto the points. 
This results in point-wise projections of dimension $\mathbb{R}^{V\times1}$ for SAM and $\mathbb{R}^{V\times384}$ for Dinov2, where $V$ is the number of viewpoints per chunk and 384 is the Dinov2 feature dimension. 
To retrieve the final Dinov2 feature vector, the point-wise projections are averaged over all viewpoint $V$.  
SAM instance masks are preprocessed in a manner that counteracts oversegmentation, i.e. we are merging subinstances such as windows into larger-scale instances such as cars. \CEDRIC{We do so by dropping smaller masks that have an intersection of at least $50\%$ of the smaller masks area with a larger mask. As the dropped instances are often enclosed by larger masks, we perform morphological operations to reduce noise by replacing missing labels with the ones of larger masks.} \ALEXEY{i would mention that this is really a user-adjustable threshold} \CEDRIC{added explanation, could add the formula for computing mask intersection if needed}
This feature reprojection is performed on the downsampled chunk with chunk size 0.05m but still need to be applied on the downsampled chunk with chunk size 0.35 which is input to the normalized cuts algorithm.
This is done by simply copying the feature vector of the point closest to the point in the downsampled pointcloud with voxelsize 0.35.\ALEXEY{does this mean that features are assigned to e.g. voxel centers?} \LAURENZ{yeah so right now we are just copying the features from the point that is closest to the voxel-center and disregarding all others. We could also think about doing a majority vote or an average depending on wether features are discrete or continuous}

For feature reprojection (see section \ref{2dfeatures}) we downsample the non-ground chunk with a smaller voxelsize of 0.05m, preserving large detail in the point cloud, and having the right density (not too dense and not too sparse) to perform mesh-based hidden points removal.\LAURENZ{This leads to points clouds of sizes between $1-2 \times 10^5$. The voxelsize has empirically shown to be a good trade-off between good HPR results and reasonable time for label reprojection} 



\paragraph{Building the Proxy-Graph}
For each downsampled chunk independently, we construct an instance-based proxy-graph where nodes correspond to points in the downsampled chunk and edges describe similarity scores between pairs of nodes. 
Edges connecting points outside a fixed spatial proximity of $\tau_{\text{spat.}} = 1$\,m\todo{explain} are assigned zero weight.

We define the final weight $w_{\text{total}}(p, q)$ between the nodes $p$ and $q$ according to a multiplicative rule to evenly integrate contributions of individual feature components into the total edge connectivity:
\begin{equation}
w_{\text{total}} = 
w_{\text{spat.}} \times
w_{\text{point}} \times
w_{\text{image}}
\end{equation}
where factors are define above.



The normalized sum-of-mismatches distance for SAM labels is computed by\ALEXEY{is this similar to edit-distance on strings? would be nice to give intuition what this measures} \LAURENZ{generally this just measures the number of instance-mismatches for two points over all viewpoints. The only changes applied to this is, that we are just counting mismatches when both points are actually visible (i.e. not -1) and that we are normalizing over the number of viewpoints where both points are visible}

    \begin{equation}
        d_{SAM}(a,b)=\frac{\sum_{i=1}^n \delta\left(a_i \neq b_i \& \&\left(a_i \neq-1 \text { or } b_i \neq-1\right)\right)}{\sum_{i=1}^n \delta\left(a_i \neq-1 \& \& b_i \neq-1\right)}
    \end{equation}

where the entry -1 refers to no label, which generally means that a point was hidden due to HPR and $\delta$ is the Kronecker Delta that returns 1 if True and 0 otherwise.




\paragraph{Performing Normalized Cuts}

The proxy graph from section \ref{graph} is input to the normalized cut algorithm based on \cite{shi2020normalized} with a maximum cutting threshold of T = XY \LAURENZ{The algorithm produces segments of points that we consider as instance proxy-labels. Those per-point instance labels are input to our deep learning architecture.}
\ALEXEY{unfinished section?} \LAURENZ{Is that enough? Or should I explain the general functioning of the normalized cuts?}


==> src/main/old/03.3-self-training.tex <==
 \subsection{Self-Training of Improved 3D Instances}
\label{method:overview}

3D instance masks obtained in~\cref{sec:instance-prop} provide an instance-based scene description but can include noisy or spurious detections as seen in ~\cref{fig:method-overview}.
Instead of treating them as final instances, similarly to recent 3D scene understanding approaches~\cite{rozenberszki2023unscene3d,zhang2023freepoint,zhang2023towards}, we seek to improve these initial predictions by passing them to a NN \textit{self-trained} to arrive at a more optimal instance segmentation. 

Let $\mathcal{M}_{pseudo}$ denote the set of 3D instance masks produced by the Normalized Cuts \cite{shi2000normalized} algorithm. 
We regard $\mathcal{M}_{pseudo}$, the output of our pseudo-instances generation step, as machine-generated pseudo-ground-truth labels used to bootstrap the training procedure. This initial set of pseudo masks often over- or undersegments objects in the scene as visualized in ~\cref{fig:method-overview}. As demonstrated by previous works \cite{ye2021learning}, during the training process neural networks tend to first learn clean labels, before fitting to the noisy data samples \cite{arpit2017closer}. To exploit this we generate a dataset of pseudo-labeled point clouds by running our Normalized Cuts \cite{shi2000normalized} algorithm. Due to the significant density of our aggregated chunk-based point clouds, we preprocess our chunks using uniform downsampling. This dataset is consequently used to train a 3D backbone \cite{marcuzzi2023mask} which learns to fit to the clean data samples, leading to the correction of over- or under-segmented instances as well as a refined ground detection. The bootstrapped network is trained for a single self-training iteration and then employed at inference time, resulting in an improved instance segmentation when compared to the initial pseudo-labels. 

We utilize the Panoptic Segmentation network MaskPLS~\cite{marcuzzi2023mask}, adapting it to our class-agnostic setting and train it with a combination of dice and cross-entropy losses, demonstrated by equation (3).  \ALEXEY{give a formula}  \ALEXEY{specify arguments for $L$ and other loss terms} In equation (3) $L_{Dice}$ and $L_{BCE}$ represent the Dice and Binary Cross Entropy Loss respectively and  $\lambda_{Dice}$ and $\lambda{BCE}$ are the weight of the loss terms. 

\begin{equation}
\label{eq:self-training-loss}
L =\lambda_{Dice} \cdot L_{Dice} + \lambda_{BCE} \cdot L_{BCE}
\end{equation}





